Combinatorics of the Permutahedra, Associahedra, and Friends

I present an overview of the research I have conducted for the past ten years in algebraic, bijective, enumerative, and geometric combinatorics. The two main objects I have studied are the permutahedron and the associahedron as well as the two partial orders they are related to: the weak order on permutations and the Tamari lattice. This document contains a general introduction (Chapters 1 and 2) on those objects which requires very little previous knowledge and should be accessible to non-specialist such as master students. Chapters 3 to 8 present the research I have conducted and its general context. You will find: * a presentation of the current knowledge on Tamari interval and a precise description of the family of Tamari interval-posets which I have introduced along with the rise-contact involution to prove the symmetry of the rises and the contacts in Tamari intervals; * my most recent results concerning q, t-enumeration of Catalan objects and Tamari intervals in relation with triangular partitions; * the descriptions of the integer poset lattice and integer poset Hopf algebra and their relations to well known structures in algebraic combinatorics; * the construction of the permutree lattice, the permutree Hopf algebra and permutreehedron; * the construction of the s-weak order and s-permutahedron along with the s-Tamari lattice and s-associahedron. Chapter 9 is dedicated to the experimental method in combinatorics research especially related to the SageMath software. Chapter 10 describes the outreach efforts I have participated in and some of my approach towards mathematical knowledge and inclusion.

==> includes/figures/decomp-interval-posets/I1.tex <==

\begin{tikzpicture}[scale=.8]
\node(T1) at (0,0) {1};
\end{tikzpicture}

==> includes/figures/decomp-interval-posets/v2.tex <==

\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 2, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\end{tikzpicture}

==> includes/figures/decomp-interval-posets/v4.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\begin{tikzpicture}[scale=0.9]
\node(T1) at (0,0) {1};
\node(T3) at (1,-1) {3};
\node(T2) at (1,0) {2};
\node(T4) at (3,0) {4};
\node(T5) at (2,-1) {5};
\node(T6) at (3,-1) {6};
\node(T7) at (4,-1) {7};
\node(T8) at (4,-2) {8};
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\draw[line width = 0.5, color=blue] (T2) -- (T4);
\draw[line width = 0.5, color=blue] (T3) -- (T4);
\draw[line width = 0.5, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=blue] (T6) -- (T7);
\draw[line width = 0.5, color=red] (T8) -- (T7);
\draw[line width = 2, color=red] (T5) -- (T4);
\draw[line width = 2, color=red] (T6) -- (T4);
\end{tikzpicture}

==> includes/figures/decomp-interval-posets/v5.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\begin{tikzpicture}[scale=1]
\node(T1) at (-1,-1) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T4) -- (T3);
\end{tikzpicture}


==> includes/figures/decomp-interval-posets/v7.tex <==

\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 2, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\end{tikzpicture}

==> includes/figures/dtrees/F022_1.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle,fill=red!50] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodef  \& \nodeg  \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(c) edge (d) edge (f) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}


==> includes/figures/dtrees/F022_2.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=red!50] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodeg  \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/F022_3.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=red!50] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle,fill=white] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle,fill=red!50] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodee  \& \nodeg  \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d) edge (e)
	(f) edge (g)
	(a) edge (b) edge (f) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/F022_inter.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodeg  \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/F10.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=red!50] (b) {$8$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$5$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=red!50] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle,fill=red!50] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle,fill=red!50] (ba) {$1$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$3$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle,fill=red!50] (bh) {$6$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle,fill=red!50] (bj) {$2$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodef  \&         \&         \&         \&         \& \nodeg  \&         \& \nodecd \\ 
         \& \nodec  \&         \&         \& \nodeh  \&         \&         \&         \& \nodebh \& \nodecc \&         \\ 
 \noded  \&         \& \nodee  \& \nodei  \&         \&         \& \nodej  \& \nodebi \& \nodebj \& \nodecb \&         \\ 
         \&         \&         \&         \& \nodeba \&         \& \nodebc \& \nodebg \& \nodeca \&         \&         \\ 
         \&         \&         \&         \& \nodebb \& \nodebd \& \nodebe \& \nodebf \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d) edge (e)
	(b) edge (c)
	(ba) edge (bb)
	(bc) edge (bd) edge (be) edge (bf)
	(j) edge (ba) edge (bc) edge (bg)
	(h) edge (i) edge (j)
	(bj) edge (ca)
	(bh) edge (bi) edge (bj) edge (cb)
	(g) edge (h) edge (bh) edge (cc)
	(a) edge (b) edge (f) edge (g) edge (cd);
\end{tikzpicture}}

==> includes/figures/dtrees/F10_2.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle,fill=white] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=red!50] (e) {$8$}
;}\newcommand{\nodef}{\node[draw,circle,fill=red!50] (f) {$7$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle,fill=white] (i) {$9$}
;}\newcommand{\nodej}{\node[draw,circle,fill=red!50] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle,fill=white] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle,fill=red!50] (bb) {$3$}
;}\newcommand{\nodebc}{\node[draw,circle,fill=red!50] (bc) {$1$}
;}\newcommand{\nodebd}{\node[draw,circle,fill=white] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle,fill=white] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle,fill=white] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle,fill=white] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle,fill=white] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle,fill=red!50] (bi) {$6$}
;}\newcommand{\nodebj}{\node[draw,circle,fill=white] (bj) {$$}
;}\newcommand{\nodeca}{\node[draw,circle,fill=red!50] (ca) {$2$}
;}\newcommand{\nodecb}{\node[draw,circle,fill=white] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle,fill=white] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle,fill=white] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \&         \& \nodee  \&         \&         \&         \&         \& \nodei  \&         \&         \& \nodecd \\ 
 \nodec  \&         \& \noded  \&         \& \nodef  \&         \&         \& \nodej  \&         \& \nodebh \&         \& \nodebi \&         \\ 
         \&         \&         \& \nodeg  \&         \& \nodeh  \& \nodeba \& \nodebb \& \nodebg \&         \& \nodebj \& \nodeca \& \nodecc \\ 
         \&         \&         \&         \&         \&         \& \nodebc \& \nodebe \& \nodebf \&         \&         \& \nodecb \&         \\ 
         \&         \&         \&         \&         \&         \& \nodebd \&         \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(f) edge (g) edge (h)
	(e) edge (f)
	(bc) edge (bd)
	(bb) edge (bc) edge (be) edge (bf)
	(j) edge (ba) edge (bb) edge (bg)
	(ca) edge (cb)
	(bi) edge (bj) edge (ca) edge (cc)
	(i) edge (j) edge (bh) edge (bi)
	(a) edge (b) edge (e) edge (i) edge (cd);
\end{tikzpicture}}

==> includes/figures/dtrees/F10_inter.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle,fill=white] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$8$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle,fill=white] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle,fill=red!50] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle,fill=white] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle,fill=white] (bb) {$3$}
;}\newcommand{\nodebc}{\node[draw,circle,fill=white] (bc) {$1$}
;}\newcommand{\nodebd}{\node[draw,circle,fill=white] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle,fill=white] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle,fill=white] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle,fill=white] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle,fill=white] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle,fill=red!50] (bi) {$6$}
;}\newcommand{\nodebj}{\node[draw,circle,fill=white] (bj) {$$}
;}\newcommand{\nodeca}{\node[draw,circle,fill=red!50] (ca) {$2$}
;}\newcommand{\nodecb}{\node[draw,circle,fill=white] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle,fill=white] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle,fill=white] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodee  \&         \&         \&         \& \nodeg  \&         \&         \&         \& \nodecd \\ 
 \nodec  \&         \& \noded  \& \nodef  \& \nodeh  \&         \&         \& \nodebh \&         \& \nodebi \&         \&         \\ 
         \&         \&         \& \nodei  \&         \& \nodej  \&         \&         \& \nodebj \& \nodeca \& \nodecc \&         \\ 
         \&         \&         \&         \& \nodeba \& \nodebb \& \nodebg \&         \&         \& \nodecb \&         \&         \\ 
         \&         \&         \&         \& \nodebc \& \nodebe \& \nodebf \&         \&         \&         \&         \&         \\ 
         \&         \&         \&         \& \nodebd \&         \&         \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(e) edge (f)
	(bc) edge (bd)
	(bb) edge (bc) edge (be) edge (bf)
	(j) edge (ba) edge (bb) edge (bg)
	(h) edge (i) edge (j)
	(ca) edge (cb)
	(bi) edge (bj) edge (ca) edge (cc)
	(g) edge (h) edge (bh) edge (bi)
	(a) edge (b) edge (e) edge (g) edge (cd);
\end{tikzpicture}}

==> includes/figures/dtrees/T05.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$4$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$ $}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$ $}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \\ 
 \nodeb  \&         \& \nodec  \\
};

\path[ultra thick, red] (a) edge (b) edge (c);
\end{tikzpicture}}

==> includes/figures/dtrees/T10_example_pure_max.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$8$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$5$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$7$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$9$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$4$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$3$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$1$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$6$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$2$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeg  \&         \&         \& \nodej  \&         \&         \&         \&         \\ 
         \&         \& \noded  \& \nodeh  \&         \& \nodei  \& \nodeba \& \nodebb \&         \&         \& \nodebj \&         \\ 
         \& \nodee  \&         \& \nodef  \&         \&         \& \nodebc \& \nodebd \& \nodebi \& \nodeca \& \nodecb \& \nodecc \\ 
         \&         \&         \&         \&         \&         \& \nodebe \& \nodebg \& \nodebh \&         \&         \& \nodecd \\ 
         \&         \&         \&         \&         \&         \& \nodebf \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e) edge (f)
	(c) edge (d)
	(g) edge (h) edge (i)
	(be) edge (bf)
	(bd) edge (be) edge (bg) edge (bh)
	(bb) edge (bc) edge (bd) edge (bi)
	(cc) edge (cd)
	(bj) edge (ca) edge (cb) edge (cc)
	(j) edge (ba) edge (bb) edge (bj)
	(a) edge (b) edge (c) edge (g) edge (j);
\end{tikzpicture}}

==> includes/figures/dtrees/T10_example_pure_max2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$9$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$8$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$4$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$3$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$1$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$6$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$2$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodee  \&         \&         \&         \& \nodef  \&         \&         \& \nodebj \&         \\ 
 \nodec  \&         \& \noded  \&         \& \nodeg  \&         \&         \& \nodeba \& \nodebi \& \nodeca \& \nodecb \& \nodecc \\ 
         \&         \&         \&         \& \nodeh  \&         \& \nodebb \& \nodebc \& \nodebd \&         \&         \& \nodecd \\ 
         \&         \&         \& \nodei  \&         \& \nodej  \&         \& \nodebe \& \nodebf \& \nodebh \&         \&         \\ 
         \&         \&         \&         \&         \&         \&         \&         \& \nodebg \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(h) edge (i) edge (j)
	(g) edge (h)
	(bf) edge (bg)
	(bd) edge (be) edge (bf) edge (bh)
	(ba) edge (bb) edge (bc) edge (bd)
	(f) edge (g) edge (ba) edge (bi)
	(cc) edge (cd)
	(bj) edge (ca) edge (cb) edge (cc)
	(a) edge (b) edge (e) edge (f) edge (bj);
\end{tikzpicture}}

==> includes/figures/dtrees/T10_example_pure_max_inter.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$8$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$4$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$3$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$1$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$6$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$2$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodee  \&         \&         \&         \& \nodeg  \&         \&         \& \nodebj \&         \\ 
 \nodec  \&         \& \noded  \& \nodef  \& \nodeh  \&         \&         \& \nodeba \& \nodebi \& \nodeca \& \nodecb \& \nodecc \\ 
         \&         \&         \& \nodei  \&         \& \nodej  \& \nodebb \& \nodebc \& \nodebh \&         \&         \& \nodecd \\ 
         \&         \&         \&         \&         \&         \& \nodebd \& \nodebf \& \nodebg \&         \&         \&         \\ 
         \&         \&         \&         \&         \&         \& \nodebe \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(e) edge (f)
	(h) edge (i) edge (j)
	(bd) edge (be)
	(bc) edge (bd) edge (bf) edge (bg)
	(ba) edge (bb) edge (bc) edge (bh)
	(g) edge (h) edge (ba) edge (bi)
	(cc) edge (cd)
	(bj) edge (ca) edge (cb) edge (cc)
	(a) edge (b) edge (e) edge (g) edge (bj);
\end{tikzpicture}}

==> includes/figures/dtrees/T10_example_pure_min.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$8$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$5$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$1$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$3$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$6$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$2$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodef  \&         \&         \&         \&         \&         \& \nodeg  \&         \&         \& \nodecd \\ 
         \& \nodec  \&         \&         \& \nodeh  \&         \&         \&         \&         \& \nodebh \&         \& \nodecc \&         \\ 
 \noded  \&         \& \nodee  \& \nodei  \&         \&         \& \nodej  \&         \& \nodebi \& \nodebj \& \nodecb \&         \&         \\ 
         \&         \&         \&         \& \nodeba \&         \& \nodebc \& \nodebg \&         \& \nodeca \&         \&         \&         \\ 
         \&         \&         \&         \& \nodebb \& \nodebd \& \nodebe \& \nodebf \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d) edge (e)
	(b) edge (c)
	(ba) edge (bb)
	(bc) edge (bd) edge (be) edge (bf)
	(j) edge (ba) edge (bc) edge (bg)
	(h) edge (i) edge (j)
	(bj) edge (ca)
	(bh) edge (bi) edge (bj) edge (cb)
	(g) edge (h) edge (bh) edge (cc)
	(a) edge (b) edge (f) edge (g) edge (cd);
\end{tikzpicture}}

==> includes/figures/dtrees/T25.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$ $}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$ $}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$ $}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \\ 
 \nodeb  \& \nodec  \& \noded  \\ 
         \&         \& \nodee  \\ 
         \&         \& \nodef  \\
};

\path[ultra thick, red] (e) edge (f)
	(d) edge (e)
	(a) edge (b) edge (c) edge (d);
\end{tikzpicture}}


==> includes/figures/dtrees/T5_example_cong.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$5$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$3$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$4$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$2$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$1$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \\ 
         \& \nodeb  \&         \&         \&         \&         \& \nodee  \&         \& \nodeba \\ 
 \nodec  \&         \& \noded  \&         \& \nodef  \&         \&         \& \nodei  \&         \\ 
         \&         \&         \& \nodeg  \&         \& \nodeh  \&         \& \nodej  \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(f) edge (g) edge (h)
	(i) edge (j)
	(e) edge (f) edge (i)
	(a) edge (b) edge (e) edge (ba);
\end{tikzpicture}}

==> includes/figures/dtrees/T5_example_cong_down.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$5$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$3$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$4$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \\ 
         \& \nodeb  \&         \&         \&         \&         \& \nodeh  \&         \& \nodeba \\ 
 \nodec  \&         \&         \& \noded  \&         \& \nodei  \&         \& \nodej  \&         \\ 
         \&         \& \nodee  \&         \& \nodef  \&         \&         \&         \&         \\ 
         \&         \&         \&         \& \nodeg  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (f) edge (g)
	(d) edge (e) edge (f)
	(b) edge (c) edge (d)
	(h) edge (i) edge (j)
	(a) edge (b) edge (h) edge (ba);
\end{tikzpicture}}


==> includes/figures/dtrees/T5_example_cong_up.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$5$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$3$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$4$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$2$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$1$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \&         \& \nodee  \&         \&         \& \nodeh  \&         \\ 
 \nodec  \&         \& \noded  \& \nodef  \&         \& \nodeg  \& \nodei  \&         \& \nodej  \\ 
         \&         \&         \&         \&         \&         \&         \&         \& \nodeba \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(e) edge (f) edge (g)
	(j) edge (ba)
	(h) edge (i) edge (j)
	(a) edge (b) edge (e) edge (h);
\end{tikzpicture}}


==> includes/figures/dtrees/T5_notpure1.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$5$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$4$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$3$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \& \nodea  \&         \\ 
         \&         \&         \& \nodeb  \&         \& \nodeba \& \nodebb \\ 
         \& \nodec  \&         \& \nodei  \& \nodej  \&         \&         \\ 
 \noded  \& \nodef  \& \nodeh  \&         \&         \&         \&         \\ 
 \nodee  \& \nodeg  \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(f) edge (g)
	(c) edge (d) edge (f) edge (h)
	(b) edge (c) edge (i) edge (j)
	(a) edge (b) edge (ba) edge (bb);
\end{tikzpicture}}

==> includes/figures/dtrees/T5_notpure2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$5$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$4$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$3$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$1$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \&         \&         \& \noded  \&         \& \nodebb \\ 
 \nodec  \&         \& \nodee  \&         \& \nodei  \& \nodeba \&         \\ 
         \& \nodef  \& \nodeg  \& \nodeh  \& \nodej  \&         \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(e) edge (f) edge (g) edge (h)
	(i) edge (j)
	(d) edge (e) edge (i) edge (ba)
	(a) edge (b) edge (d) edge (bb);
\end{tikzpicture}}

==> includes/figures/dtrees/T6_stamari.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$6$}
;}\newcommand{\nodeb}{\node[draw,circle, ,fill=red!50] (b) {$4$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$2$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$3$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$5$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \\ 
         \&         \& \nodeb  \&         \&         \&         \&         \&         \& \nodeba \&         \& \nodebd \\ 
 \nodec  \&         \& \nodee  \&         \&         \& \nodeh  \&         \& \nodebb \&         \& \nodebc \&         \\ 
 \noded  \& \nodef  \&         \& \nodeg  \& \nodei  \&         \& \nodej  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d)
	(e) edge (f) edge (g)
	(h) edge (i) edge (j)
	(b) edge (c) edge (e) edge (h)
	(ba) edge (bb) edge (bc)
	(a) edge (b) edge (ba) edge (bd);
\end{tikzpicture}}


==> includes/figures/dtrees/T6_stamari2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$6$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$5$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$4$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$2$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$3$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \&         \&         \&         \&         \&         \&         \& \noded  \&         \& \nodebd \\ 
 \nodec  \&         \&         \& \nodee  \&         \&         \&         \&         \&         \& \nodebc \&         \\ 
         \& \nodef  \&         \& \nodeg  \&         \&         \& \nodej  \&         \&         \&         \&         \\ 
         \&         \& \nodeh  \&         \& \nodei  \& \nodeba \&         \& \nodebb \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(g) edge (h) edge (i)
	(j) edge (ba) edge (bb)
	(e) edge (f) edge (g) edge (j)
	(d) edge (e) edge (bc)
	(a) edge (b) edge (d) edge (bd);
\end{tikzpicture}}

==> includes/figures/dtrees/T_012_two_facets1.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \noded  \&         \& \nodeg  \\ 
 \nodec  \& \nodee  \&         \& \nodef  \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(d) edge (e) edge (f)
	(a) edge (b) edge (d) edge (g);
\end{tikzpicture}}

==> includes/figures/dtrees/T_012_two_facets2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeg  \\ 
         \& \noded  \&         \& \nodef  \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(c) edge (d) edge (f)
	(a) edge (b) edge (c) edge (g);
\end{tikzpicture}}

==> includes/figures/dtrees/T_012_two_facets3.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$2$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \&         \&         \\ 
 \nodeb  \& \noded  \&         \& \nodee  \&         \\ 
 \nodec  \&         \& \nodef  \&         \& \nodeg  \\
};

\path[ultra thick, red] (b) edge (c)
	(e) edge (f) edge (g)
	(a) edge (b) edge (d) edge (e);
\end{tikzpicture}}

==> includes/figures/dtrees/T_012_two_facets4.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$2$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \&         \&         \\ 
 \nodeb  \& \nodec  \&         \& \nodee  \&         \\ 
         \& \noded  \& \nodef  \&         \& \nodeg  \\
};

\path[ultra thick, red] (c) edge (d)
	(e) edge (f) edge (g)
	(a) edge (b) edge (c) edge (e);
\end{tikzpicture}}


==> includes/figures/dtrees/T_012_two_facets5.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeg  \\ 
 \nodec  \&         \& \nodee  \&         \&         \\ 
 \noded  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d)
	(b) edge (c) edge (e)
	(a) edge (b) edge (f) edge (g);
\end{tikzpicture}}

==> includes/figures/dtrees/T_012_two_facets6.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeg  \\ 
 \nodec  \&         \& \noded  \&         \&         \\ 
         \&         \& \nodee  \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(b) edge (c) edge (d)
	(a) edge (b) edge (f) edge (g);
\end{tikzpicture}}

==> includes/figures/dtrees/T_012_two_facets7.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodee  \& \nodeg  \\ 
 \nodec  \&         \& \noded  \& \nodef  \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(e) edge (f)
	(a) edge (b) edge (e) edge (g);
\end{tikzpicture}}

==> includes/figures/dtrees/T_012_two_facets8.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeg  \\ 
         \& \noded  \&         \& \nodee  \&         \\ 
         \&         \&         \& \nodef  \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e)
	(a) edge (b) edge (c) edge (g);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_example1.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$ $}
;}\newcommand{\noded}{\node[draw,circle] (d) {$ $}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$2$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$ $}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$ $}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$ $}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \&         \&         \\ 
 \nodeb  \& \noded  \&         \& \nodee  \&         \\ 
 \nodec  \&         \& \nodef  \& \nodeg  \& \nodeh  \\
};

\path[ultra thick, red] (b) edge (c)
	(e) edge (f) edge (g) edge (h)
	(a) edge (b) edge (d) edge (e);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_example2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$ $}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$ $}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$ $}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$ $}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$ $}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodeg  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodef  \&         \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(b) edge (c) edge (d) edge (f)
	(a) edge (b) edge (g) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_examplejoin.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$ $}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$ $}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$ $}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$ $}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$ $}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \&         \&         \\ 
 \nodeb  \& \nodec  \&         \& \noded  \&         \\ 
         \&         \& \nodee  \& \nodef  \& \nodeh  \\ 
         \&         \&         \& \nodeg  \&         \\
};

\path[ultra thick, red] (f) edge (g)
	(d) edge (e) edge (f) edge (h)
	(a) edge (b) edge (c) edge (d);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_two_facets1.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodeg  \& \nodeh  \\ 
 \nodec  \& \nodee  \& \nodef  \&         \&         \\ 
 \noded  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d)
	(b) edge (c) edge (e) edge (f)
	(a) edge (b) edge (g) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_two_facets2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \noded  \&         \& \nodeh  \\ 
 \nodec  \& \nodee  \& \nodef  \& \nodeg  \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(d) edge (e) edge (f) edge (g)
	(a) edge (b) edge (d) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_two_facets3.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodef  \& \nodeg  \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(c) edge (d) edge (f) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}


==> includes/figures/dtrees/T_022_two_facets4.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodeg  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodef  \&         \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(b) edge (c) edge (d) edge (f)
	(a) edge (b) edge (g) edge (h);
\end{tikzpicture}}


==> includes/figures/dtrees/T_022_two_facets5.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodeg  \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_two_facets6.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodeg  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodee  \&         \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(b) edge (c) edge (d) edge (e)
	(a) edge (b) edge (g) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_two_facets7.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodee  \& \nodeg  \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d) edge (e)
	(f) edge (g)
	(a) edge (b) edge (f) edge (h);
\end{tikzpicture}}

==> includes/figures/dtrees/T_022_two_facets8.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodef  \&         \\ 
         \&         \&         \& \nodeg  \&         \\
};

\path[ultra thick, red] (f) edge (g)
	(c) edge (d) edge (e) edge (f)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> includes/figures/interval-posets/I2-ex1.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013


\begin{tikzpicture}[scale=0.8]
\node(T1) at (0,0) {1};
\node(T2) at (0,-1) {2};
\draw[line width = 0.5, color=red] (T2) -- (T1);
\end{tikzpicture}



==> includes/figures/interval-posets/I3-ex1.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013


\begin{tikzpicture}[xscale=0.5, yscale=0.8]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 0.5, color=red] (T3) -- (T2);
\end{tikzpicture}


==> includes/figures/interval-posets/I3-ex2.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013


\begin{tikzpicture}[xscale=0.8, yscale=0.8]
\node(T2) at (0,-1) {2};
\node(T1) at (0,0) {1};
\node(T3) at (1,-1) {3};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T2) -- (T1);
\end{tikzpicture}


==> includes/figures/interval-posets/I3-ex3.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013


\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\draw[line width = 0.5, color=red] (T3) -- (T2);
\end{tikzpicture}


==> includes/figures/interval-posets/I3-ex4.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}

\node(N1) at (0,\hlev) {1};
\green{
\node(T1) at (0,0) {2};
\node(T2) at (0,-1) {3};
\draw[line width = 0.5, color=red] (T2) -- (T1);
}
\end{tikzpicture}


==> includes/figures/interval-posets/I3-ex5.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}

\node(N1) at (0,\hlev) {1};
\green{
\node(T1) at (0,0) {2};
\node(T2) at (0,-1) {3};
\draw[line width = 0.5, color=red] (T2) -- (T1);
}
\draw[line width = 0.5, color=red](T1) -- (N1);
\end{tikzpicture}


==> includes/figures/interval-posets/I4-ex1.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\begin{tikzpicture}[scale=1]
\node(T1) at (-1,-1) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T4) -- (T3);
\end{tikzpicture}


==> includes/figures/interval-posets/I4-ex2.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}[scale=0.8]
\node(T2) at (0,-1) {2};
\node(T1) at (0,0) {1};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T2) -- (T1);
\draw[line width = 0.5, color=red] (T4) -- (T3);
\end{tikzpicture}



==> includes/figures/interval-posets/I6-ex1.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013
\def \hlev{0.8}
\def \wlev{0.6}

\begin{tikzpicture}
\node(N1) at (0,0) {1};
\node(N2) at (0.5 * \wlev,-1 * \hlev) {2};
\node(N3) at (\wlev,0) {3};
\node(N4) at (2 * \wlev,0) {4};
\node(N5) at (3 * \wlev,0) {5};
\node(N6) at (3 * \wlev,-1 * \hlev) {6};
\draw (N2) -- (N3);
\draw (N2) -- (N1);
\draw (N6) -- (N5);
\end{tikzpicture}


==> includes/figures/interval-posets/I6-ex3.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013


\begin{tikzpicture}[scale=0.8]
\node(T2) at (0,-1) {2};
\node(T1) at (0,0) {1};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\node(T5) at (2,-2) {5};
\node(T6) at (2,-3) {6};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T2) -- (T1);
\draw[line width = 0.5, color=red] (T6) -- (T5);
\end{tikzpicture}


==> includes/figures/interval-posets/I6-ex6.tex <==


\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (1,0) {3};
\node(T4) at (2,0) {4};
\node(T5) at (1,-1) {5};
\node(T6) at (2,-1) {6};
\draw[line width = 0.5, color=blue] (T1) -- (T3);
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=blue] (T3) -- (T4);
\draw[line width = 0.5, color=blue] (T5) -- (T6);
\end{tikzpicture}

==> includes/figures/relations/r2_0.tex <==
\begin{tikzpicture}[baseline, scale=\interscale]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\draw[->,line width = 0.5, color=white, opacity=0] (T1) edge [bend left=70] (T2);
\draw[->,line width = 0.5, color=white, opacity=0] (T2) edge [bend left=70] (T1);
\end{tikzpicture}

==> includes/figures/relations/r3_0.tex <==
\begin{tikzpicture}[baseline, scale=\interscale]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (2,0) {3};
\draw[->,line width = 0.5, color=white, opacity=0] (T1) edge [bend left=70] (T3);
\draw[->,line width = 0.5, color=white, opacity=0] (T3) edge [bend left=70] (T1);
\end{tikzpicture}

==> includes/figures/relations/r3_12.tex <==
\begin{tikzpicture}[baseline, scale=\interscale]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (2,0) {3};
\draw[->, line width = 0.5, color=blue] (T1) edge [bend left=70] (T2);
\draw[->,line width = 0.5, color=white, opacity=0] (T1) edge [bend left=70] (T3);
\draw[->,line width = 0.5, color=white, opacity=0] (T3) edge [bend left=70] (T1);
\end{tikzpicture}

==> includes/figures/relations/r3_23.tex <==
\begin{tikzpicture}[baseline, scale=\interscale]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (2,0) {3};
\draw[->, line width = 0.5, color=blue] (T2) edge [bend left=70] (T3);
\draw[->,line width = 0.5, color=white, opacity=0] (T1) edge [bend left=70] (T3);
\draw[->,line width = 0.5, color=white, opacity=0] (T3) edge [bend left=70] (T1);
\end{tikzpicture}

==> includes/figures/relations/r3_32.tex <==
\begin{tikzpicture}[baseline, scale=\interscale]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (2,0) {3};
\draw[->, line width = 0.5, color=red] (T3) edge [bend left=70] (T2);
\draw[->,line width = 0.5, color=white, opacity=0] (T1) edge [bend left=70] (T3);
\draw[->,line width = 0.5, color=white, opacity=0] (T3) edge [bend left=70] (T1);
\end{tikzpicture}

==> includes/figures/trees/T2-1.tex <==
% Auteur : Viviane Pons
% Création : 11/05/2013

%     .
%   ./

\begin{tikzpicture}
\node (N0) at (0.750, 0.000){};
\node (N00) at (0.250, -0.500){};
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T2-2.tex <==
% Auteur : Viviane Pons
% Création : 29/05/2013

%     .
%      \.

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N00) at (0.750, -0.500){};
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T3-1-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T3-1.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.750, -0.500){};
\node (N000) at (0.250, -1.000){};
\draw[Point] (N000) circle;
\draw (N00.center) -- (N000.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T3-2-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T3-2.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.250, -0.500){};
\node (N001) at (0.750, -1.000){};
\draw[Point] (N001) circle;
\draw (N00.center) -- (N001.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T3-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T3-3.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (1.250, -0.500){};
\node (N010) at (0.750, -1.000){};
\draw[Point] (N010) circle;
\draw (N01.center) -- (N010.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T3-4-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T3-4.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (0.750, 0.000){};
\node (N00) at (0.250, -0.500){};
\draw[Point] (N00) circle;
\node (N01) at (1.250, -0.500){};
\draw[Point] (N01) circle;
\draw (N0.center) -- (N00.center);
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T3-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T3-5.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (0.750, -0.500){};
\node (N011) at (1.250, -1.000){};
\draw[Point] (N011) circle;
\draw (N01.center) -- (N011.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> includes/figures/trees/T4-1-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%      /
%     /
%    /

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (1.500, -2.000){2};
\node (N0000) at (0.500, -3.000){1};
\draw (N000) -- (N0000);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-10-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%      ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\node (N0100) at (1.500, -3.000){2};
\draw (N010) -- (N0100);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-11-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%         \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (1.500, -2.000){2};
\node (N0101) at (2.500, -3.000){3};
\draw (N010) -- (N0101);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-12-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%         \.
%        ./ \.
%        

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N010);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-13-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%           \.
%          ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (3.500, -2.000){4};
\node (N0110) at (2.500, -3.000){3};
\draw (N011) -- (N0110);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-14-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%         \.
%           \.
%             \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\node (N0111) at (3.500, -3.000){4};
\draw (N011) -- (N0111);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-2-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./
%     \

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (0.500, -2.000){1};
\node (N0001) at (1.500, -3.000){2};
\draw (N000) -- (N0001);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./\.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\node (N001) at (2.500, -2.000){3};
\draw (N00) -- (N000);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-4-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%       \.
%      ./

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (2.500, -2.000){3};
\node (N0010) at (1.500, -3.000){2};
\draw (N001) -- (N0010);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%      ./
%       \.
%        \.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\node (N0011) at (2.500, -3.000){3};
\draw (N001) -- (N0011);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> includes/figures/trees/T4-6-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%     ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-7-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%       \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-8-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%        ./

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\draw (N01) -- (N010);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> includes/figures/trees/T4-9-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%           \.

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N011);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}
